Dipolar physics: A review of experiments with magnetic quantum gases

Since the achievement of quantum degeneracy in gases of chromium atoms in 2004, the experimental investigation of ultracold gases made of highly magnetic atoms has blossomed. The field has yielded the observation of many unprecedented phenomena, in particular those in which long-range and anisotropic dipole-dipole interactions play a crucial role. In this review, we aim to present the aspects of the magnetic quantum-gas platform that make it unique for exploring ultracold and quantum physics as well as to give a thorough overview of experimental achievements.

==> Section7/10_conclusions.tex <==
\section{Perspectives}

The present time is highly exciting for research based on magnetic atoms.  Many substantial advances are being made at an impressively rapid pace. %brought forward at an impressively fast pace. 
New experimental apparatus are coming online soon and promise to bring even more excitement. %and the novel possibility offered by state-of-the-art setups will shed new lights on many unexplored issues. 
State-of-the-art techniques, recently implemented in other ultracold-atom experiments, will soon become available in lanthanide experiments.   These promising to shed new light on the physics that has been revealed within the few last years.  For example, single-atom  `quantum gas' microscopes are well-poised to reveal additional details regarding the strong correlations of the many-body states that have been observed both in bosonic and fermionic dipolar quantum gases as well as open the way to extend investigations of their far-from-equilibrium dynamics. Control on the single-atom level will also provide novel understanding, at the few-body level, of scattering phenomena in these complex lanthanide systems. Complete magnetic shielding will enable the exploration of the zero-field regime of spin physics. Exploiting the rich optical transition spectrum of the lanthanides will also provide novel capabilities for controlling spins and interactions more exquisitely. The prospect of realising topological quantum states is one of many central aims. 

Highly versatile trap geometries will also play a role and provide new prospects for exploring the interplay between the anisotropic and long-range character of the DDI and the geometry of the system.  Other ingredients, such as disorder and frustration could also be added to the systems.  The mixture of different magnetic and non-magnetic species will reveal new physics, and in particular,  could provide access to dipolar physics with an internal degree of freedom and distinct dipolar moments but without dipolar relaxation. Mass imbalance effects could also be explored. This opens new avenues toward exotic few-body as well as many-body phenomena, including Efimov states, $p$-wave superfluidity, and other exotic states of matter. One cannot capture all the possible new directions enabled by highly magnetic atoms, but undoubtedly, brand-new physics will arrive in the next years, and we hope for new surprises to match those this review has presented.



\subsection*{Acknowledgements}

All the authors would like to warmly thank their countless collaborators over the years, both from the experiment and for the theory sides. They were all crucial actors to the discoveries summarised in this review. Additionally, we are grateful to Steven Lepoutre, Fabian Boettcher, Wil Kao, and Kuan-Yu Li for their careful reading of the manuscript. 
L.C., I.F.B., F.F., and T.P.  acknowledge the support from the international collaborative network on dipolar quantum gases funded by the DFG and FWF - FOR 2247/PI2790. F.F., B.L.T., and T.P. acknowledge support through the QuantERA grant MAQS. 
L.C. acknowledges support by the Deutsche Forschungsgemeinschaft (DFG, German Research Foundation) under
Germany’s Excellence Strategy EXC 2181/1-390900948 (the Heidelberg STRUCTURES Excellence Cluster) and Project-ID No. 273811115 (SFB1225 ISOQUANT). 
B.L.T acknowledges support from CNRS, Conseil Régional d’Ile-de-France under SIRTEQ Agency, and Agence Nationale de la Recherche (Project
No. ANR-18-CE47-0004).
B.L.L. acknowledges support from the NSF and AFOSR. T.P acknowledges support from the European Research Council (ERC)  (Grant agreement No. 101019739).
